Inverse problems in spin models

Several recent experiments in biology study systems composed of several interacting elements, for example neuron networks. Normally, measurements describe only the collective behavior of the system, even if in most cases we would like to characterize how its different parts interact. The goal of this thesis is to extract information about the microscopic interactions as a function of their collective behavior for two different cases. First, we will study a system described by a generalized Ising model. We find explicit formulas for the couplings as a function of the correlations and magnetizations. In the following, we will study a system described by a Hopfield model. In this case, we find not only explicit formula for inferring the patterns, but also an analytical result that allows one to estimate how much data is necessary for a good inference.

==> introduction.tex <==
\begin{itemize}
\item Aim of the thesis: extract useful information from overwhelming 
amount of data produced in recent biological experiments
\end{itemize}
\section*{Outline of the thesis}

%% \begin{itemize}
%% \item Review of experiments in biology where underlying system is composed of
%% multiple interacting units and we can measure the state of its individual
%% components.
%% \item Review and discussion of some models of neural networks
%% \item Review of previous work on inverse models in statistical mechanics
%% \item Analytical expansion for small couplings
%% \item Hopfield model, short review and discussion (fixed-rang matrix 
%% expansion for the $J_{ij}$ matrix, potentially meaningful patterns)
%% \item Theoretical limits in quantity of data needed for inference in Hopfield 
%% model
%% \item Pattern inference in Hopfield model
%% \end{itemize}



